3D-OES: Viewpoint-Invariant Object-Factorized Environment Simulators

We propose an action-conditioned dynamics model that predicts scene changes caused by object and agent interactions in a viewpoint-invariant 3D neural scene representation space, inferred from RGB-D videos. In this 3D feature space, objects do not interfere with one another and their appearance persists over time and across viewpoints. This permits our model to predict future scenes long in the future by simply "moving" 3D object features based on cumulative object motion predictions. Object motion predictions are computed by a graph neural network that operates over the object features extracted from the 3D neural scene representation. Our model's simulations can be decoded by a neural renderer into2D image views from any desired viewpoint, which aids the interpretability of our latent 3D simulation space. We show our model generalizes well its predictions across varying number and appearances of interacting objects as well as across camera viewpoints, outperforming existing 2D and 3D dynamics models. We further demonstrate sim-to-real transfer of the learnt dynamics by applying our model trained solely in simulation to model-based control for pushing objects to desired locations under clutter on a real robotic setup

==> oldexp.tex <==
\section{Experiments}\label{sec:experiments}


We evaluate \ES\ on its prediction accuracy for single- and multi-step object motion forecasting under multi-object interactions, as well as on its performance in model predictive control for pushing objects to desired locations on a table surface in the presence of obstacles. We perform controlled ablations to test the generalization of our model under varying camera viewpoints, varying number and appearance of objects present. 



We train  our model to predict 3D object motion during robot objects pushing and objects falling in the Bullet Physics Simulator. For \textbf{pushing}, we collect data of objects moving while pushed by a Kuka robotic arm and record RGB-D video streams from multiple viewpoints. We create scenes using 31 different 3D object meshes, including 11 objects from the MIT Push dataset \citep{mitpush} and 20 objects selected from four categories (\textit{camera}, \textit{mug}, \textit{bowl} and \textit{bed}) in the ShapeNet Dataset \citep{shapenet2015}. At training time each scene contains at most two (potentially interacting) objects. For \textbf{falling}, we use 3D meshes of the objects introduced in \cite{DBLP:journals/corr/abs-1812-10972}, including a variety of shapes. We randomly select 1-3 objects and initialize their positions by placing them on the table surface, and let one object fall freely from the above. For both \textbf{pushing} and \textbf{falling}, we train out model with three camera views, and use either three or one randomly selected views as input during test time.  
 


% \textbf{\textit{Baselines}}
We compare \ES\ against a set of baselines chosen to capture representative models of the existing literature on object dynamics:
%, trying to group related work into a few distinct models.
%We compare our model against the following baselines: 

\todo{did we use any public code for the things below???}
\begin{enumerate}
    \item \Bone, that mimics Interaction Networks  \citep{DBLP:journals/corr/BattagliaPLRK16} and \citep{DBLP:journals/corr/abs-1808-00177, WuLuKohli17}. It is a graph neural network where object features are the 3D object centroid locations and their velocities, and edge features the relative 3D locations,
    %as object state, and incorporate cross-object interactions for forecasting motions using a graph network, similar to . 
    \item \Btwo, identical to the one used in \Bone. It is a graph neural network over 3D object centroid locations and object-centric 2D image feature embeddings that  forecasts 3D object rotations and translations. \todo{??This model extracts 2D CNN features and combine them with camera pose and 3D object centroid before feeding into a graph network}.

    \item 
    Visual Foresight (\textit{VF}) of \cite{ebert2018visual}, a model that uses the current frame and the action of the agent to predict future 2D frames by ``moving pixels" based on predicted 2D pixel flow fields.
   
    \item 
    \Pla \cite{hafner2019planet}, a model that learns a scene-level embedding by predicting future frames and the reward given the current frame. 
    %The model then performs planning in latent space to select the actions to execute.

    \end{enumerate} 
For further details of data collection, train-test split, and implementation details of the baselines, please refer to Appendix.
We compare our model against baselines \Bone \ and \Btwo \  on both motion forecasting and model predictive control. Since \VF \ and \Pla \ work in 2D image space and do cannot use them to predict 3D object motion, we thus compare against them for performing pushing with model predictive control.

\begin{table}[h!]
\centering
\caption{\textbf{Motion prediction error of pushing objects in scenes with two objects} for 1,3, and 5 timestep prediction horizon. We show prediction error using different number of views as inputs.
%^training and testing under randomly selected novel views. 
}
\begin{tabular}{c|l|cccc}
            \multicolumn{1}{l|}{Experiment Setting}          & 
            \multicolumn{1}{l|}{Model}          & 
            \multicolumn{1}{l}{}          & 
            \multicolumn{1}{l}{T=1} & \multicolumn{1}{l}{T=3} &  \multicolumn{1}{l}{T=5}
            \\ \hline
3views (randomly selected, novel)  &\Bone~  

\citep{DBLP:journals/corr/BattagliaPLRK16,DBLP:journals/corr/abs-1808-00177, WuLuKohli17}& translation(mm) 
                 & $4.6$ & $32.1$  & $66.3$  \\
       + gt-bbox &      & rotation(degree) 
                 & $2.8$ & $16.7$ & $26.4$\\
                 &\Btwo  &translation(mm)  
                 & $6.0$& $39.3$& $69.7$\\
                 &      & rotation(degree) 
                 &$3.4$ & $29.8$  & $30.7$  \\
                 &Ours  &translation(mm)
                 & ${\bf 3.6}$ & $ {\bf 22.5}$ & ${\bf 43.4}$ \\
                 &      & rotation(degree) 
                & ${\bf 2.5}$ & ${\bf 12.0}$ & ${\bf 20.6}$ \\\hline
1view (randomly selected, novel) &\Btwo  &translation(mm)  
                 & $6.0$& $39.3$& $69.7$\\
     + gt-bbox           &      & rotation(degree) 
                 &$3.4$ & $29.8$  & $30.7$  \\
                 &Ours  &translation(mm)
                 &  ${\bf 4.1}$ & ${\bf 23.6}$ & ${\bf 43.8}$ \\
                 &      & rotation(degree) 
                & ${\bf 3.1}$ & ${\bf 12.2}$ & ${\bf 20.3}$ \\\hline
1view (randomly selected, novel) &\Bone ~  
\citep{DBLP:journals/corr/BattagliaPLRK16,DBLP:journals/corr/abs-1808-00177, WuLuKohli17}& translation(mm) 
                 & 6.7 & 35.4 & 68.2  \\
                 + predicted-bbox from GRNNs  &      & rotation(degree) 
                 & 3.0 & 20.1 & 30.32 \\
                 &\Btwo  &translation(mm)  
                 & $6.6$& $43.1$& $71.2$\\
                 &      & rotation(degree) 
                 &$3.6$ & $31.8$  & $32.4$  \\
                 &Ours  &translation(mm)
                 & ${\bf 4.3}$& ${\bf 25.2}$& ${\bf 47.0}$\\
                 &      & rotation(degree) 
                 & ${\bf 2.7}$ & ${\bf 12.1}$ & ${\bf 19.7}$  \\\hline
1view (fixed, same as training) 
                 &\Btwo  &translation(mm)  
                 & $5.1$& $29.6$ & $54.5$\\
+ predicted-bbox from GRNNs 
                 &      & rotation(degree) 
                 & $2.6$ & $11.0$ & $16.9$ 
               \\\hline
\end{tabular}


\label{tab:2obj}
\end{table}


\begin{table}[h!]
\caption{\textbf{Motion prediction error of falling objects in scenes with three to four objects} for 1,3, and 5 timestep prediction horizon.
%^training and testing under randomly selected novel views. 
}
\centering
\begin{tabular}{c|l|cccc}
            \multicolumn{1}{l|}{Experiment Setting}          & 
            \multicolumn{1}{l|}{Model}          & 
            \multicolumn{1}{l}{}          & 
            \multicolumn{1}{l}{T=1} & \multicolumn{1}{l}{T=3} &  \multicolumn{1}{l}{T=5}
            \\ \hline
1views (randomly selected, novel)  &\Bone ~  

\citep{DBLP:journals/corr/BattagliaPLRK16,DBLP:journals/corr/abs-1808-00177, WuLuKohli17} & translation(mm) 
                 & $5.2 $ & ${\bf 11.7}$  & $278.6$  \\
       + predicted-bbox &      & rotation(degree) 
                 & $ {\bf 5.7} $ & $ {\bf 10.4} $ & $ 43.28 $\\
                 &\Btwo  &translation(mm)  
                 & $8.4$& $17.0$& $620.2$\\
                 &      & rotation(degree) 
                 &$9.2$ & $16.6$  & $117.9$  \\
                 &Ours  &translation(mm)
                 & ${\bf 5.0}$ & $ 13.1$ & ${\bf 16.4}$ \\
                 &      & rotation(degree) 
                & $ 6.1$ & $ 12.6 $ & ${\bf 18.7}$ \\\hline
\end{tabular}


% \vspace{-20pt}
\label{tab:2obj_fall}
\end{table}

\subsection{Action-Conditioned 3D Object Motion Forecasting}
We evaluate performance of our model and the baselines in single- and multi-step 3D motion forecasting for \textbf{pushing} and \textbf{falling} in Tables \ref{tab:2obj} and \ref{tab:2obj_fall} in terms of translation and rotation error. 
We ablate by i) using 1 or 3 camera views at the first time step, ii) using goundtruth 3D object boxes (gt-bbox) or 3D boxes predicted by the detector. 
\todo{None of the objects are seen during training.} 
Our model outperforms the  baselines both in translation and rotation prediction accuracy. When tested with object boxes predicted by the 3D object detector (Section \ref{sec:enc}) as opposed to ground-truth 3D boxes, our model is the least affected. \Btwo \  performs on par with or even worse than \Bone, indicating that it does not gain from having access to additional appearance information.  We hypothesize this is due to the way appearance and camera pose information are integrated in this model: the model simply treats camera pose information as additional input, similar to  \cite{ye2019objectcentric}, as opposed to our model, which leverages geometry-aware representations that retain the geometric structure of the scene.


\textbf{Multi-step forward unrolling} The \Bone \  baseline can be easily  unrolled  forward in time without  much error accumulation since it does not use any appearance features. Still, our model outperforms it. Though our model uses appearance features in the form of 3D object-centric feature maps, it uses  appearance temporal skip connections to minimize error accumulation over time.  In contrast, \Bone \ is oblivious to the appearance of the object and thus cannot effectively adapt its predictions to different object shapes.
 
 
\textbf{Varying number of camera views} 
 Our model  accepts a variable number of  views as input, and improves when more views are available; yet, it can accurately predict future motion even from a single view. The prediction error of our single view model is only slightly higher than the model using three random views as input.  As shown in Table \ref{tab:2obj}, the \Btwo \  baseline performs the worst and does not improve with more views available. We believe this is due to the geometry-unaware way of combining multiview information by concatenation, though the model does have access to camera poses of the input images. Indeed, we show in Table \ref{tab:2obj} (last 2 rows) that \Btwo \  can achieve much higher performance when \textbf{trained and tested on a single fixed camera viewpoint}. This is a setting widely used in the recently popular learning-based visual-motor control literature \cite{DBLP:journals/corr/FinnL16, pathakICLR18zeroshot, ye2019objectcentric, ebert2018visual}, which though restricts the corresponding models to  work only under carefully controlled environments, while  ours performs competitively to the 2D model with fixed camera viewpoint but can handle arbitrary camera viewpoint. %, and can easily break during occlusions.



%\todo{keep or not keep} Additionally, we conducted another experiment where we test our model's performance over varing end-effector geometries. We train our model in the 2-obj scene, using only the single rod Kuka robot as the pushing agent for data collection, and then test the model on pushing tasks using robot with 6 different end-effectors with varying geometries (see the appendix for the detailed designs). Interestingly, as shown in Table \ref{tab:singlestep_2obj} row 2, our model is able to generalize well to novel end-effector design although it's only trained on a simple rod-shape end-effector, since it captures such dynamics by learning inter-object interactions, where the objects provide geometry diversities.




%\end{figure*}



%\paragraph{Inferring 3D object detections for object-centric dynamics????}
%Most previous works on learning object-centric dynamic models assume object segmentations given, i.e., they assume the state of the simulator known, and they focus on approximating its next-step function. However, accurately detecting objects in 3D  is an unsolved problem, and given the projection artifacts and occlusions in the input RGB stream, 3D object detection is as difficult as, if not more difficult, than applying learned dynamics over ground-truth 3D boxes. The architectures we propose invert the input RGB stream to obtain a stable 3D feature model of the scene. Such architectures are ideal for extracting 3D object detections that persist over time despite occlusions \citep{commonsense}. In Table \ref{tab:detection_1obj}, we show motion prediction performance using the 3D object detector built on top of the 3D latent representation. Our model outperforms all the baselines, and reaches comparable results as the one using groudtruth object poses.
\textbf{Varying number of objects, novel scenes}
In Figure \ref{fig:rollout}, we qualitatively show 2 samples of long term motion prediction results produced by unrolling our model forward in time (more are shown in the supplementary video). We test the models trained with three input views and two-object scenes with varying numbers of views and objects. It can be seen our model generalizes to novel objects and scenes with varying number of objects, though only 2 objects are present in the scene during training. \todo{THIS IS NOT EXPLAINED, THAT THIS IS A RNEDER OF 3D MESHES BASED ON PREDICTED MOTIONS,.}
We can  visualize the latent 3D feature map by neurally projecting it from a camera viewpoint and decoding the projection into an image through a learned neural decoder. In Appendix Section A.1, we show  interpretable RGB images are rendered using the learned neural image decoder. 



\begin{figure*}[t!]
	\centering
		\centering
		\includegraphics[width=1.0\textwidth]{figures/rollout_predictions4.png}
		%\hline
	%	\includegraphics[width=1.0\textwidth]{figures/rollout_2.pdf}
		\caption{{\bf Forward unrolling of our dynamics model and the \Bone\  baseline.} Left: pushing. Right: falling.
		In the top row, we show (randomly sampled) camera  views that we use as input to our model. %,  randomly selected from the 27 locations (9 different azimuths and 3 different elevations). 
		The second row shows the ground-truth motion of the object from the front view. 
		%Note that the model might not see any image from this view; this is just for visualization. 
		Rows 3, 4 show the predicted object motion from our model and the \Bone \  baseline from the same front camera viewpoint. Notice that our model matches more accurately the ground-truth object motion than the \Bone \  baseline. The latter is oblivious to object appearance.
		%\todo{does this use predicted boxes or gt?}% overhead camera.  %Our model shows a clear performance margin over the baselines.
		%		The plot shows precision-recall curves for all methods, with a 3D intersection-over-union threshold of 0.5. Contrastive learning outperforms all baselines.
		}
			\label{fig:rollout}
	%\caption{Precision-recall curves on 3D object detectionwith a moving camera}
\end{figure*}
%\subsection{Ablation study on the proposed modules}
%\todo{* compare with 3d object-centric features with graph network.
%* compare with explicit update, but no order-graph interaction network.
%}

\vspace{-0.1in}
\subsection{Counterfactual Simulations}
The proposed \ES\ not only can simulate the future state of the scene, but it can also imagine counterfactuals: we can freely move and rotate objects
in the scene neural map to  new positions by simply cutting-and-pasting its features from its original place to the target position, and then run \ES\ to predict the future trajectory of such scene variations.  
In Section A.2 of the supplementary material, we  show multiple counterfactual simulations resulting from enlarging  objects or moving them around, and then simulating the corresponding outcomes with \ES\.


\vspace{-0.1in}
\subsection{Pushing with Model Predictive Control (MPC)}
We test the performance of our model with MPC to push objects to desired locations and report the results in Table \ref{tab:control}. For our model and \Btwo, we use a single randomly sampled view. For \VF \ and \Pla, we use a fixed top-down view for both training and testing as they only work with a fixed viewpoint. We use planning horizon of 1 step since greedy action selection suffices for this task. Note that longer planning horizon is needed for planning collision-free path with obstacles in the scene, as shown later. Details of the experiment setting are included in Appendix (Section C.3).


\begin{table}[t!]
\caption{Success rate for pushing objects to target locations. }
\centering
\begin{tabular}{c c c c c|c}
            \multicolumn{1}{l}{\Bone ~  
\citep{DBLP:journals/corr/BattagliaPLRK16,DBLP:journals/corr/abs-1808-00177, WuLuKohli17}}        &  \multicolumn{1}{l}{\Btwo} & \multicolumn{1}{l}{\VF \cite{ebert2018visual }  & \multicolumn{1}{l}{\Pla \cite{hafner2019planet} }  &
            \multicolumn{1}{l|}{Ours} &\multicolumn{1}{l}{Ours-Real}  \\ \hline
0.76 & 0.70  & 0.32 & 0.16& ${\bf 0.86}$ & 0.78 \\
\end{tabular}
\label{tab:control}
\end{table}
%We compare our model against baselines in Table \ref{tab:control}.
%. Our model performs 
% and final 







%In Figure \ref{fig:rollout}, we show the results. Our model can predict reasonable outcomes for as long as five times steps and the results are qualitatively better than the baseline models, both in single step prediction and multi-steps prediction. 






%\subsection{Multi-step prediction on unseen objects}
%In Figure \ref{fig:rollout_unseen}, we show multi-step prediction results on unseen objects. Our model can better generalize to unseen objects than the baselines.







%We compare our 3D object detector with a  detector  that given an RGB frame predicts the centroid $(X,Y,Z)$ of the 3D bounding box for the object using a series of convolutional and fully connected layers, used recently in \cite{DBLP:journals/corr/abs-1808-00177}. We show the Mean Average Precision (mAP) for both models in Table \ref{tab:detection}. We see that our architecture much outperforms the baseline. 


% \vspace{-20pt}
Our model outperforms all baselines by a great margin. We also train and test variants of \VF \ and \Pla \ to take observations from varying camera viewpoints, together with camera pose information. However, they both fail completely on this task.

\textbf{Collision-free pushing}
In order to test our model's multi-step prediction performance, we evaluate our model on pushing in scenes with randomly sampled obstacles, and the robot is required to push an object to desired goals without colliding into any obstacle.
For quantitative evaluation, we randomly place an object of interest and a goal position in the planar workspace. One obstacle is placed between them with a small perturbation, so that there exists no straight collision-free path to reach the goal. We achieve a success rate of $\mathbf{0.68}$ for this task. See Appendix (Section C.3) for further details of the experiment setting.

Since randomly placing multiple obstacles in the scene for quantitative evaluation while ensuring existence of collision-free path is non-trivial, we show qualitative planning results for such complex scenes in the supplementary video.

\vspace{-0.1in}
\paragraph{Sim-to-Real Transfer}
We train our  model  in simulation and test  it  on object pushing control task in a real  Baxter platform equipped with a rod-shaped end-effector, similar to the setting in the Bullet simulation. We attached a Intel RealSense D435 RGB-D camera to the robot's left hand, and use only one RGB-D view as input for this experiment. The pose of the camera is different from those seen during  training. Please, see Section C.3 of the supplementary file for details of our real-world setup, objects selection, and 3D detector training. 
We report the success rate of real world pushing in Table \ref{tab:control} (Ours-Real). Our model achieves similar success rates for pushing  in simulation and in the real world, showing good sim-to-real transferability. 
 We attribute this to the good transferability of the 3D scene feature representations, that do not suffer from projection artifacts and can match across viewpoints.  In the supplementary material, we include a video showing model-predictive pushing control of objects along collision-free trajectories in complex scenes on the real-world setup.
%Since geometry information is shared by simulation and the real world by a large extent, and our model combines the view-invariant property of the geometry-aware representation and an object-factorized structure, it presents good sim-to-real transferrability. 
%We also qualitatively evaluate pushing with collision-avoidance in complex scenes on the real-world setup, and show planned action sequences in the supplementary video.

\begin{comment}


\begin{table}[h!]
\centering
\begin{tabular}{c|cccccc}
            \multicolumn{1}{l|}{}          &
            \multicolumn{1}{l}{$\mathrm{mAP}_{0.33}^{d}$}          &  \multicolumn{1}{l}{$\mathrm{mAP}_{0.50}^{d}$} & \multicolumn{1}{l||}{$\mathrm{mAP}_{0.75}^{d}$} &  \multicolumn{1}{l }{$\mathrm{mAP}_{0.33}^{m}$} & \multicolumn{1}{l}{$\mathrm{mAP}_{0.50}^{m}$} &
            \multicolumn{1}{l}{$\mathrm{mAP}_{0.75}^{m}$} \\  \hline
\cite{DBLP:journals/corr/abs-1808-00177} &  $ 0.817$ & $0.654$ & $0.165$  & - & -& -  \\
ours & ${\bf 0.923}$ & ${\bf 0.813}$  & ${\bf 0.280}$  & $0.866$  & $0.757$ & $0.154$\\
\end{tabular}
\caption{Mean Average Precision (mAP) for 3D object detection and 3D segmentation for three different thresholds of Intersection over Union (IoU) (0.75,0.5,0.33)}
\label{tab:detection}
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{c|c|cccc}
            \multicolumn{1}{l|}{}& 
            \multicolumn{1}{l|}{Experiment Setting} & 
            \multicolumn{1}{l}{\Bone} & \multicolumn{1}{l}{\Btwo} &  \multicolumn{1}{l}{\Bthree} & \multicolumn{1}{l}{ours}
            \\ \hline
object position (mm) & 3views + gt-bbox  & $13.9$ & $13.9$  & $8.30$  & ${\bf 7.12}$ \\
object orientation (degree) &  & $10.3$ & $11.7$  & $3.90$  & ${\bf 3.94}$  \\ \hline
object position (mm) & 3views + gt-bbox  & $19.4$ & $23.2$  & $13.6$  & ${\bf 12.5}$ \\
object orientation (degree) & + varfinger  & $11.4$ & $12.8$  & ${\bf 4.06}$  & $ 4.07$  \\ \hline
\end{tabular}
\caption{Single step prediction error with  \textbf{multiple objects}. We evaluate the models with fingertips of various shape.}
\label{tab:singlestep_2obj}
\end{table}

\end{comment}

% \subsection{Discussion - Limitations} \label{sec:limitations}
%\todo{marrying 3D perception and control, maybe we should mention this earlier too?}
%Our model combines 3D perception and dynamics learning in a 3D feature space inferred from the RGB-D stream. 

%The ability to detect objects in 3D at test time is critical the for success of our object-centric  3D motion forecaster as well as control framework that relies on estimating free space for collision avoiding object trajectories. 
%Most previous works on object-centric dynamic models assume 2D object segmentations given  or easily obtainable from color segmentation of the video frames \cite{DBLP:journals/corr/abs-1812-10972,Wu_2017_CVPR}. However, accurately detecting objects in 3D  is an unsolved problem, and given the projection artifacts and occlusions in the input RGB stream, 3D object detection is as difficult as, if not more difficult, than applying learned dynamics over ground-truth 3D boxes. The model we propose marries 3D perception and control by detecting objects and estimating their dynamics in the 3D feature bottleneck of inverse graphics networks %. %The architectures we propose inverts the input RGB stream to obtain a stable 3D feature model of the scene %. 
%Such architectures are ideal for extracting 3D object detections that persist over time despite occlusions 
%\citep{commonsense}, pursuing a 3D feature representation instead of explicit ones such as meshes, pointclouds or voxel occupancies, trained end-to-end for 3D object detection and 3D object dynamics learning.  


% Our model currently has  three main limitations:
% \textbf{(i)} It uses strong  supervision at training time regarding object 3D locations and relative 3D rotations. Automatically inferring 3D tracking of objects during interactions from neurally projecting in 2D the inferred 3D feature maps warped under the  estimated 3D rotations and translations  and backpropagating the frame prediction  error is a direct avenue of future work that would permit our  model to be trained in a  self-supervised manner for frame prediction in non-instrumented environments. 
% \textbf{(ii)} It assumes rigid object interactions by capturing future object motion in 3D rotations and translations. Learning dynamics of soft bodies and fluids would require  forecasting a general dense 3D flow field, and potentially a residual appearance 3D feature change that  predicted motion  cannot account for. We will pursue this direction using simulators that permit simulation of soft bodies and fluids \cite{DBLP:journals/corr/abs-1810-05762}. 
% \textbf{(iii)} It learns deterministic dynamics. Adding stochasticity to prediction using  stochastic neural networks \cite{kingma2013auto,liu2016stein}  for predicting object's motion, or exploring motion-contrastive objectives \citep{DBLP:journals/corr/abs-1807-03748} is a direct avenue for future work. 


%We leave all these extensions for future work. 




\begin{comment}

%\begin{figure*}[h!]
\begin{figure*}[h!]
\centering
\begin{tabular}{c|l|cccc}
            \multicolumn{1}{l|}{Experiment Setting}          & 
            \multicolumn{1}{l|}{Model}          & 
            \multicolumn{1}{l}{}          & 
            \multicolumn{1}{l}{T=1} & \multicolumn{1}{l}{T=3} &  \multicolumn{1}{l}{T=5}
            \\ \hline
3views (randomly selected, novel)  &\Bone & translation(mm) 
                 & $4.6$ & $32.1$  & $66.3$  \\
 + gt-bbox       &      & rotation(degree) 
                 & $2.8$ & $16.7$ & $26.4$\\
                 &\Btwo  &translation(mm)  
                 & $6.0$& $39.3$& $69.7$\\
                 &      & rotation(degree) 
                 &$3.4$ & $29.8$  & $30.7$  \\
                 &\Bthree &translation(mm)
                 & $3.8$ & ${\bf 22.2}$ & ${\bf 42.8}$ \\
                 &      & rotation(degree) 
                 & $2.6$ & ${\bf 12.0}$ &  $20.8$  \\
                 &Ours  &translation(mm)
                 & ${\bf 3.6}$ & $ 22.5$ & $ 43.4$ \\
                 &      & rotation(degree) 
                & ${\bf 2.5}$ & ${\bf 12.0}$ & ${\bf 20.6}$ \\\hline
1view (randomly selected, novel) &\Btwo  &translation(mm)  
                 & $6.0$& $39.3$& $69.7$\\
      + gt-bbox  &      & rotation(degree) 
                 &$3.4$ & $29.8$  & $30.7$  \\
                 &\Bthree &translation(mm)
                 & ${\bf 3.8}$ & $24.2$ & $44.0$ \\
                 &      & rotation(degree) 
                 & $3.3$ & $12.3$ &  $20.4$  \\
                 &Ours  &translation(mm)
                 &  $4.1$ & ${\bf 23.6}$ & ${\bf 43.8}$ \\
                 &      & rotation(degree) 
                & ${\bf 3.1}$ & ${\bf 12.2}$ & ${\bf 20.3}$ \\\hline
1view (randomly selected, novel) &\Bone & translation(mm) 
                 & 6.7 & 35.4 & 68.2  \\
                 + predicted-bbox from GRNNs  &      & rotation(degree) 
                 & 3.0 & 20.1 & 30.32 \\
                 &\Btwo  &translation(mm)  
                 & $6.6$& $43.1$& $71.2$\\
                 &      & rotation(degree) 
                 &$3.6$ & $31.8$  & $32.4$  \\
                 &\Bthree &translation(mm)
                 & $4.4$ & ${\bf 24.7}$ & $47.3$  \\
                 &      & rotation(degree) 
                 & $2.8$ & $13.4$ & $20.3$  \\
                 &Ours  &translation(mm)
                 & ${\bf 4.3}$& $25.2$& ${\bf 47.0}$\\
                 &      & rotation(degree) 
                 & ${\bf 2.7}$ & ${\bf 12.1}$ & ${\bf 19.7}$  \\\hline
1view (fixed, same as training) 
                 &2D-singleview  &translation(mm)  
                 & $5.1$& $29.6$ & $54.5$\\
+ predicted-bbox from GRNNs 
                 &      & rotation(degree) 
                 & $2.6$ & $11.0$ & $16.9$ 
               \\\hline
\end{tabular}
\caption{Prediction error with 2 objects. We show prediction error using different number of views as inputs.}
\label{tab:2obj}
\end{figure*}

\end{comment}

==> oldmodel.tex <==
\section{Object-Factorized Environment Simulators (3D-OES)}
%\todo{Mention:1. we chop trajectories based on timesteps, 2. we train for unrolling so the features learn to persist!
%}
\label{sec:model}
\begin{figure*}[t]
	\centering
		\centering
		\includegraphics[width=0.85\textwidth]{figures/fig2_arch.png}
		\caption{
		\textbf{3D Flow Interaction Network} for predicting 3D object motion under agent-object and object-object interactions.
		 %Input to our model are one or more RGB-D images of the scene. These are unprojected, oriented taking into account the camera viewpoints, and integrated into a set of 3D scene feature maps $\Mt \in \mathbb{R}^{w \times h \times d \times c}$  using geometry-aware recurrent  networks (GRNNs) of \cite{commonsense}.  A 3D object detector detects 3D object boxes and 3D object binary voxel occupancy masks  using the scene 3D feature $\Mt$ as input. 
		 %We then predict motion for each object detected in the scene using ordered object graph interaction layer.
		 The ordering of the object nodes is decided on the fly, but the first object is the one located in smallest Euclidean distance to the gripper. For each object, we crop $\Mt$ using the detected 3D object box to obtain $\Mt^o$.  The  object-centric feature map, $\M^o$, is concatenated with the predicted object occupancy mask and a 3D scene flow field that encodes moving objects and the moving robot gripper, and is mapped to the future 3D relative rotation and translation of the object in the next time step. 
		 Then, we transform the predicted 3D motion into a 3D flow tensor and aggregate it to the 3D flow field, to be used for the next object prediction.
		}
			\label{fig:model}
\end{figure*}

%\subsection{Learning Environment Simulators in an implicit 3D Visual Feature space}
%The architecture of our model is depicted in Figure \ref{fig:model}.  
Given a single RGB-D image or a set of posed  RGB-D images of a static scene, our model constructs a 3D scene feature representation by neurally lifting image and depth maps to feature voxel grids (Section \ref{sec:enc}). Then, it detects objects in 3D in the inferred  scene representation. Using the object-factorized scene representation, the model then predicts the future 3D rotation and translation   for each object present using an graph network module that form nodes using object-centric feature maps and passes messages between objects (Section \ref{sec:forecast}). We will assume for now rigid objects, and we  discuss in Section \ref{sec:conclusion} how to extend our framework to  deformable and articulated  objects. Actions provided by the agent are represented by the translational movement of the agent's end-effector. 


\textbf{\ES\  simulates future or counterfactual scenes by decoupling appearance and motion of the objects}. 3D appearance remains  constant  over time while motion changes. Our model composes  scenes by
warping  object appearances inferred from the input images based on predicted cumulative  3D object motion (Section \ref{sec:unroll}).  These composed 3D feature maps, though not directly interpretable, can be decoded to RGB images from any desired camera viewpoints via a neural renderer.
%(Section \ref{sec:viewpred}). 
We use long-term simulations of \ES\  to generate  action plans for pushing objects to desired locations in cluttered environments using model predictive control (Section \ref{sec:control}).  
%For completeness, we start  by describing previous work on GRNNs  \cite{commonsense} that is the perceptual front end of the proposed simulation model, in Section \ref{sec:GRNN}.

%\section{View Invariant Object Factorized Environment Simulators (3DOES}

%We consider two datasets, push dataset and falling-object dataset.

We train our model to learn dynamics of objects being pushed on a table surface and objects falling on top of others.  
%The push dataset includes random robot-object interactions where our robot pushes the objects on a table surface. The falling-object dataset includes trajectory of an object falling on other objects. The agent is not moving in the second dataset. 
%For each 3D scene, we assume we can sample camera viewpoints and observe the corresponding 2D RGB-D images.
At training time, we  assume access  to  3D object bounding boxes to train our 3D object detector. 
 %In Section \ref{sec:forecast}, we describe the proposed view-invariant object-factorized environment simulator model. 
 %In Section \ref{sec:unroll}, we describe unrolling of our model forward in  time to predict long term effects of actions, or effects of actions sequences. 

\subsection{Differentiable 2D-to-3D lifting by  Geometry-Aware Recurrent Networks (GRNNs)}
\label{sec:enc}
Geometry-Aware Recurrent Networks (GRNNs) introduced in \cite{commonsense,adam3d} learn to ``lift" RGB-D images of static  world scenes to  3D scene feature maps while being optimized  end-to-end for a downstream task, such as supervised 3D object detection or unsupervised view prediction.   GRNNs are equipped with trainable  neural modules that map   between 2D pixel space and 3D feature space in a differentiable manner.   
   %They are  inspired by Simultaneous Localization and Mapping (SLAM) methods \cite{sturm12iros}, but instead of 3D pointcloud maps they build 3D feature maps. These feature maps are not the final output, but rather the \textit{bottleneck} of the network architecture. Thus, such feature maps can represent a wide variety of information that is related to the downstream task, as opposed to merely 3D  occupancy 
   We will denote the 3D scene feature   as $\M \in \mathbb{R}^{w \times h \times d \times c}$ where $w,h,d,c$ denote width, height, depth and number of channels, respectively. %, i.e., the inferred 3D feature maps, when projected from designated camera viewpoints, are neurally decoded to  2D RGB images whose pixel values should be close to the corresponding ground-truth RGB image view. 
 Every $(x, y, z)$ grid location in the 3D feature map $\M$ holds an  1-dimensional feature vector  that  describes the semantic and geometric properties of a corresponding 3D physical location in the 3D world scene. 
 %necessary for achieving the downstream task.  
 The  map is  updated with each new video frame by estimating egomotion and  transforming the features accordingly to cancel the estimated egomotion before updating the map in a convolutional manner; in this way,    information from 2D pixels that correspond to the same 3D physical point end up nearby in the map. In our case, we need such cross-frame registration in case we have access to concurrent multiple views for the first timestep of the simulation. 
 %GRNNs are end-to-end differentiable.  %At training time, we assume a mobile agent that  moves around in a 3D world scene and sees it from multiple camera viewpoints, in order to provide ``labels" for view prediction to GRNNs. 
     Upon training, GRNNs  map  RGB-D images or a single RGB-D image to a  \textit{complete} 3D feature map of the scene they depict, i.e., the model learns to \textit{imagine} the missing or occluded information. We denote this 2D-to-3D mapping as $\M=\Enc(I_1, ..., I_t), \M \in \mathbb{R}^{W \times H \times D \times c} $. Note that the input can be a single RGB-D image, in which case $\M=\Enc(I)$.   For further details on GRNNs, please refer to \cite{commonsense,adam3d}. 
     
     

     
\noindent \textbf{3D object detection }
  A 3D detector operates on the output of the encoder $\Enc$ and predicts a variable number of object boxes with corresponding 3D segmentation masks, i.e., binary voxel occupancies:  $\mathcal{O}=\Det(\M), \mathcal{O} =\{\hat{b}^o=(p^o_x,p^o_y,p^o_z,w^o,h^o,d^o)\in \mathbb{R}^6, m^o \in \{0,1\}^{w^o \times h^o \times d^o}, o=1 \cdots |\mathcal{O}| \}$, where $p^o_x,p^o_y,p^o_z$ stands for the 3D box centroid and $w^o,h^o,d^o$ stands for 3d box size. Its architecture is similar to Mask R-CNN \cite{DBLP:journals/corr/HeGDG17} but uses 3D input and output instead of 2D. We crop the 3D scene feature map $\M$ given a detected box to obtain an object-centric feature tensor $\M^o$. 
  
  
%Given images  annotated with 3D object boxes and 3D binary occupancy masks, we train GRNNs  to map the 3D feature map $\M$  to category-agnostic  3D bounding boxes and corresponding 3D segmentation masks for the objects present. We use    an architecture similar to 
 %the state-of-the-art 2D object detector Mask-RCNN \cite{DBLP:journals/corr/HeGDG17} that has though 3D input and output instead of 2D, as suggested by \cite{commonsense}. 
 %We use the same architecture for our category-agnostic 3D object detector   in Section \ref{sec:forecast}.  % Because the  3D feature map $\M$ is not affected by instantaneous object  occlusions and dis-occlusions caused by camera motion or changes of the camera's motion and field-of-view, detected objects persist over time, despite occlusions in the pixel observations stream. 
%Given a bounding box $b^o$ predicted by the 3D detector at the first time step, we crop the scene 3D feature representation $\M$ and obtain an object centric feature tensor $\M^o$. 

%The object-centric 3D feature map $\M_t^o$ is obtained by cropping the scene 3D feature map $\M_t$ using a fixed-size axis-aligned 3D bounding box around the predicted 3D object centroid (predicted by the 3D object detector). 

\noindent   \textbf{View prediction for visualizing  latent 3D simulations}
  We   train the encoder and decoder of our architecture end-to-end for RGB view regression as proposed in \cite{commonsense}, in order to visualize the latent scene simulations. Our decoder involves a differentiable 3D-to-2D projection that projects the 3D scene feature representation after orienting it to the query camera viewpoint. The projected features are then decoded into images through the learned decoder. \ES\  run video predictions in a latent 3D space and thus 2D RGB videos of the latent 3D simulations can be decoded from any desired viewpoints. 
  
  
  %They showed strong 
  
  %depicted in Figure \ref{fig:model} by predicting RGB views, following  work of \cite{adam3d}
  
  %\cite{commonsense} proposed a differentiable 3D-to-2D mapping which projects the 3D feature maps to 2D feature maps according to a query camera viewpoint. A neural decoder then takes the 2D features maps and decodes it into an RGB image that describes how the scene looks if we see it from the query viewpoint. The neural decoder, along with the 3D feature map, are trained under a view prediction loss that tries to minimize distance between the predicted image and the image collected by a moving agent. By training a neural decoder for our model, we can visualize and interpret the latent features learned by our model.








\subsection{Mental Simulation by Warping Persistent Object Feature Maps} \label{sec:unroll} 
Our motion forecasting module (Section \ref{sec:forecast}) predicts the 3D motion of each object for a single time step conditioned on the agent's actions and the surrounding context of object interactions. \ES\  then synthesize the scene of the next timestep  by simply warping object tensors $\M^o,o=1 ...|\mathcal{O}|$ of the first timestep to their predicted 3D locations and orientations.  
To predict long term results of action sequences, the model needs to be unrolled forward in time by feeding its predictions back as input. 
To synthesize scene of timesteps further into the future, \ES\  warp  object tensors of the first timestep---as opposed to the ones obtained from the simulated scene of the previous timestep---based on cumulative 3D motion predictions. %the initial 3D object appearance represented as the object-centric 3D feature map of the first time step $\M_0^o$, as opposed to the one computed in the last time step.
Specifically, given predicted 3D object motions ($\delta \hat{p}_t$, $\delta \hat{r}_t$) at unrolling step $t$, we estimate the \textbf{cumulative} 3D rotation and translation of the object with respect to the first timestep:
\begin{align}
    &\hat{p}_0=0 \ \ \hat{\rot}_0 = 0 \\
&\hat{p}_t=\hat{p}_{t-1}+\delta \hat{p}_t, \ \   
\hat{\rot}_t=\hat{r}_{t-1}+\delta \hat{\rot}_t , \ \   t=1 \cdots T, 
\end{align}
where $T$ denotes the number of unrolling steps thus far. 
Then, given 3D object segmentation masks $m^o$ and object-centric 3D feature maps $\M^o$ obtained by the 3D object detector from the input RGB-D images, we rotate and translate the object masks and   feature maps  using the cumulative 3D rotation $\hat{\rot}_t$ and 3D translation $\hat{p}_t$  using  3D dense spatial transformers. We  synthesize a new 3D scene feature map $\bar{\M}_{t}$ by adding each transformed object-centric 3D feature map at its predicted 3D location: 
\begin{align}
       & \bar{\M}_{t} = \sum_{o=1}^{|\mathcal{O}|} \mathrm{Draw}(\mathrm{Rotate}(m^{o}, \hat{\rot}^o_t) \odot \mathrm{Rotate}(\M^{o}, \hat{\rot}^o_t), \hat{p}^o_{t}), 
\end{align}
where superscript $o$ denotes the object identity, $\mathrm{Rotate}(\cdot, r)$ denotes 3D rotation by  angle $\rot$,  $\odot$ denotes voxel-wise multiplication,  and  $\mathrm{Draw}(\M, p)$ denotes adding a tensor $\M$  at a 3D location $p$. We then crop the simulated 3D scene map $\bar{\M}_{t}$ at the predicted 3D location for each object to obtain the next input for our forecasting model:
\begin{align}
    \bar{\M}^{o}_{t} = \mathrm{Crop}(\bar{\M}_{t}, \ \ \hat{p}^o_{t}), \forall o \in O. 
\end{align}
where  $\mathrm{Crop}(\cdot, p)$ denotes cropping a tensor using a (fixed size) 3D bounding box $b_o$ centered at location $p$.
%We use the same box size for all objects so that our network can learn to interpret object sizes. 





%The appearance temporal skip connections for model unrolling we just described are possible thanks to the what-where decomposition of the proposed 3D feature scene representations, and permanence of 3D appearance. They are not possible in image-centric state encodings or 2D object-centric dynamics where visual input is contaminated by occlusions and projection artifacts.   This is a key advantage of learning  object dynamics in a 3D feature space instead of in the 2D image space: motion prediction accounts for the wide majority of scene changes. %much fewer things change over time.





%Our model thus implicitly assumes that  3D object appearance  captured in 3D feature representations  $\M_t^o$ persists across temporal motion transformations.  %As a result, 
%is entirely represented by the 3D rotation and 3D translation it undergoes as a result of the (optional) pushing action. 
%Such appearance constancy holds exactly in 3D for most rigid or deforming objects, but only approximately in 2D due to object occlusions and dis-occlusions and size changes caused by camera zooms. This is a key advantage of learning  object dynamics in a 3D feature space instead of in the 2D image space: much fewer things change over time.

%its appearance tensor $\M_0^o$ obtained from the initial timestep according to the cumulative 3D motion of timestep $t$.

%Though representations \M are non interpre 

%of the robots  predict the future state of a scene by instantiating 3D object feature tensors 
%Our dynamics model learns to predict 3D  motion of the next timestep for each of the objects in the scene.



%Our dynamics module predicts the single step 3D motion of an object conditioned on the agent's actions and the surrounding object interactions. % for one time step. 
%To predict long term results of actions, or results of long action sequences, the model is unrolled forward in time by feeding its predictions back as input. Such  model unrolling is notorious for causing error accumulation over time  \citep{DBLP:journals/corr/abs-1011-0686}, since, at each time step, the result exhibits a small prediction error, which gets exacerbated as it is fed back as input. 



\subsection{Graph Neural Networks on Top of Object-Centric 3D Feature Maps for Object Motion Forecasting} \label{sec:forecast}

%\todo{why we predict motion}
\ES\ are equipped with an object motion forecasting module that predicts 3D  motion for one time interval  for each  object detected in the scene. %We chop time 
%We will assume for now rigid objects, and we will discuss in Section \ref{sec:limitations} how to generalize our framework to  deformable or articulated  objects.
%It simulates the future state of each object $\M_t^o$  by warping its appearance tensor $\M_0^o$ based on the predicted 3D motion of timestep $t$.
%Our model thus implicitly assumes that  3D object appearance  captured in 3D feature representations  $\M_t^o$ persists across temporal motion transformations.  %As a result, 
%is entirely represented by the 3D rotation and 3D translation it undergoes as a result of the (optional) pushing action. 
%Such appearance constancy holds exactly in 3D for most rigid or deforming objects, but only approximately in 2D due to object occlusions and dis-occlusions and size changes caused by camera zooms. This is a key advantage of learning  object dynamics in a 3D feature space instead of in the 2D image space: much fewer things change over time. %, and most changes can be encoded by 3D motion fields. 
Objects are  the recipient of forces exercised by active agents; meanwhile, objects themselves also carry momentum and causes other objects to move. 
%and senders of forces under cross-object interactions. 
How can we model cross-object dynamic relationships in a way that generalizes under varying number of objects and arbitrary chains of interactions? 
We build a graph-based interaction network, where each node update is a single-step 3D motion prediction that takes as input a 3D feature map centered around the object of interest, $\bar{\M}_t^o$, as well as the action of the agent and motion of other objects. Message passing along the edges encodes both motions of the surround objects as well as the pair-wise relative locations of all the objects. This graph-based dynamics model predicts   3D rotation and translation of all detected objects. We use $\bar{\cdot}$ to denote predicted quantities generated by our model. %, as shown in Figure \ref{fig:intro}.  
 %Given an object-centric 3D feature crop and the action representation, our forecasting model predicts  
%the  object's 3D motion for the next time step. 
The object-centric 3D feature map $\bar{\M}_t^o$ is obtained by cropping the scene 3D feature map $\bar{\M}_t$ using a fixed-size axis-aligned 3D bounding box around the predicted 3D object centroid.
%Note that $\bar{b}_t^o$ is set to 1.5 times larger that the bounding box of the object as predicted by the detector since we want to also capture immediate visual context during motion forecasting.
We predict object motions in terms of relative rotations $\delta \hat{r}$, represeted by quaternions, and 3D translations $\delta \hat{p}$. In addition, this forecasting module is trained by forward unrolling and error of each step is back-propagated through time. More implementation details are included in Appendix.
%We train our model with regression to the desired 3D object motions. 


\begin{comment}
For every object in the scene and for each time step our motion prediction loss reads:
\begin{equation}
   \mathcal{L}(\delta \hat{p}, \delta \hat{\rot}, \delta p, \delta \rot) = \sum \limits_{t=0}^T ||\delta p_t - \delta \hat{p}_t||_1 + || \delta \rot_t -  \delta \hat{\rot}_t ||^2,  \nonumber
\end{equation}
where $\delta p$ and $\delta r$ stand for the ground-truth 3D object translation and rotation, respectively. $T$ is the sequence length during training. In all our experiments, $T$ is set to $5.$
\end{comment}





%\todo{is that correct?}


\subsection{Model Predictive Control with \ES}
\label{sec:control}
Action-conditioned  simulation models, such as \ES, mentally simulate the  results of an agent's actions and permit successful control in zero-shot setups: achieving a specific  goal in a novel scene without previous practice. 
We demonstrate applying our model to a pushing task in a cluttered environment with model predictive control. Given an input RGB-D image $I$ that contains  multiple objects, a goal configuration is given in terms of the desired 3D location of an object $\x_{goal}^o$. 
%Our ability to manipulate a scene critically depends on such mental simulators, a.k.a. models of world dynamics or intuitive physics \cite{}. They 
%The use of me
%We use our model to push objects towards desired locations on the table surface.
\ES\ infer the scene 3D feature map $\M=\Enc(I)$ and detect the objects present in the  scene. We then unroll the model  forward in time using randomly sampled action sequences, as described in Section \ref{sec:unroll}.  
We evaluate each action sequence based on the Euclidean distance of the predicted location $\hat{x}^o_T$ (after $T$ time steps) for the designated object. We execute the first action of the best action sequence and repeat  \citep{tassa2008receding}. %This look-ahead multi-step planning allows us to plan desired action sequence for reaching goal locations while avoiding obstacles.
%\todo{we dont mention the collision free trajectories and waypoints ehre}
Our model combines 3D perception and planning using learned object dynamics in the inferred 3D feature space. %It uses basic spatial reasoning in the inferred 3D space to compute collision-free trajectories.
While most previous works choose bird's eye viewpoints to minimize cross-object or robot-object occlusions \cite{fang2019dynamics}, our control framework \textbf{can use any camera viewpoint}, thanks to its ability  to map input 2.5D images to complete, viewpoint invariant  3D scene feature maps. We empirically validate this claim in our experiments.



